Where Is the Flux Going? The Long-Term Photometric Variability of Boyajian's Star

We present ~800 days of photometric monitoring of Boyajian's Star (KIC 8462852) from the All-Sky Automated Survey for Supernovae (ASAS-SN) and ~4000 days of monitoring from the All Sky Automated Survey (ASAS). We show that from 2015 to the present the brightness of Boyajian's Star has steadily decreased at a rate of 6.3 +/- 1.4 mmag yr^-1, such that the star is now 1.5% fainter than it was in February 2015. Moreover, the longer time baseline afforded by ASAS suggests that Boyajian's Star has also undergone two brightening episodes in the past 11 years, rather than only exhibiting a monotonic decline. We analyze a sample of ~1000 comparison stars of similar brightness located in the same ASAS-SN field and demonstrate that the recent fading is significant at >99.4% confidence. The 2015-2017 dimming rate is consistent with that measured with Kepler data for the time period from 2009 to 2013. This long-term variability is difficult to explain with any of the physical models for the star's behavior proposed to date.

==> asas_data_table.tex <==
\begin{deluxetable}{lcc}
\tablecaption{ASAS Photometry of Boyajian's Star}
\tablewidth{0pt}
\tablehead{
\colhead{HJD} &
\colhead{$V$} &
\colhead{$\Delta V$} \\
\colhead{} &
\colhead{[mag]} &
\colhead{[mag]} 
}
\startdata
2453887.00345 & 11.928 & 0.019 \\
2453892.97057 & 11.922 & 0.034 \\
2453897.03348 & 11.937 & 0.035 \\
2453915.01509 & 11.923 & 0.028 \\
2453916.95754 & 11.940 & 0.037 \\
2453920.95091 & 11.955 & 0.035 \\
2453928.97449 & 11.941 & 0.031 \\
2453930.97710 & 11.922 & 0.017 \\
2453932.97819 & 11.918 & 0.027 \\
2453934.97840 & 11.932 & 0.057 \\
2453939.88368 & 11.944 & 0.030 \\
2453943.93553 & 11.949 & 0.055 \\
2453947.05708 & 11.954 & 0.048 \\
2453984.00225 & 11.913 & 0.022 \\
2453988.89777 & 11.928 & 0.015 \\
2453991.91789 & 11.927 & 0.014 \\
2453997.82969 & 11.909 & 0.029 \\
2454000.84771 & 11.936 & 0.019 \\
2454007.90902 & 11.922 & 0.029 \\
2454013.90124 & 11.933 & 0.019 \\
2454017.90752 & 11.968 & 0.027 \\
2454021.81557 & 11.954 & 0.019 \\
2454023.87321 & 11.925 & 0.017 \\
2454036.75062 & 11.953 & 0.027 \\
2454038.77166 & 11.954 & 0.023 \\
2454048.80781 & 11.947 & 0.015 \\
2454050.81591 & 11.917 & 0.022 \\
2454053.71493 & 11.890 & 0.018 \\
2454057.71930 & 11.881 & 0.024 \\
2454059.75745 & 11.912 & 0.025 \\
2454061.76529 & 11.907 & 0.018 \\
2454064.72716 & 11.869 & 0.019 \\
2454066.73657 & 11.903 & 0.019 \\
2454076.73163 & 11.913 & 0.023 \\
2454078.71982 & 11.907 & 0.013 \\
2454080.71483 & 11.909 & 0.026 \\
2454082.71685 & 11.909 & 0.023 \\
2454085.70877 & 11.907 & 0.014 \\
2454088.70582 & 11.916 & 0.017 \\
2454091.69346 & 11.923 & 0.031 \\
2454093.69860 & 11.927 & 0.035 \\
2454186.11493 & 11.915 & 0.016 \\
2454190.14694 & 11.933 & 0.021 \\
2454198.10484 & 11.906 & 0.017 \\
2454211.11316 & 11.916 & 0.019 \\
2454222.05142 & 11.953 & 0.020 \\
2454225.06394 & 11.970 & 0.019 \\
2454228.07978 & 11.925 & 0.017 \\
2454239.09593 & 11.949 & 0.015 \\
2454242.05857 & 11.910 & 0.016 \\
2454245.04339 & 11.916 & 0.015 \\
2454263.05273 & 11.917 & 0.017 \\
2454267.07958 & 11.909 & 0.035 \\
2454269.04610 & 11.887 & 0.015 \\
2454271.00889 & 11.923 & 0.019 \\
2454274.05924 & 11.907 & 0.021 \\
2454276.01357 & 11.901 & 0.015 \\
2454277.97175 & 11.894 & 0.024 \\
2454299.03019 & 11.899 & 0.022 \\
2454300.94713 & 11.906 & 0.022 \\
2454304.94797 & 11.907 & 0.021 \\
2454306.99350 & 11.890 & 0.015 \\
2454309.91636 & 11.914 & 0.019 \\
2454311.95397 & 11.931 & 0.016 \\
2454314.85976 & 11.906 & 0.016 \\
2454318.90592 & 11.912 & 0.019 \\
2454322.90622 & 11.922 & 0.029 \\
2454330.88940 & 11.908 & 0.020 \\
2454473.70756 & 11.922 & 0.026 \\
2454473.72246 & 11.905 & 0.022 \\
2454473.73738 & 11.916 & 0.027 \\
2454474.69802 & 11.849 & 0.037 \\
2454474.70818 & 11.912 & 0.029 \\
2454474.72861 & 11.899 & 0.023 \\
2454478.70501 & 11.924 & 0.027 \\
2454479.72632 & 11.948 & 0.023 \\
2454480.71590 & 11.894 & 0.023 \\
2454560.10674 & 11.954 & 0.016 \\
2454561.10616 & 11.910 & 0.018 \\
2454562.11251 & 11.909 & 0.039 \\
2454564.13413 & 11.926 & 0.019 \\
2454583.08810 & 11.898 & 0.022 \\
2454594.06311 & 11.897 & 0.019 \\
2454607.11135 & 11.914 & 0.028 \\
2454608.01288 & 11.967 & 0.030 \\
2454889.16680 & 11.937 & 0.029 \\
2454890.16675 & 11.992 & 0.033 \\
2454918.14076 & 11.920 & 0.021 \\
2454993.97539 & 11.900 & 0.034 \\
2455018.89666 & 11.945 & 0.036 \\
2455021.92600 & 11.908 & 0.027 \\
2455022.88589 & 11.923 & 0.037 \\
2455043.86174 & 11.892 & 0.039 \\
2455054.02400 & 11.945 & 0.021 \\
2455076.78482 & 11.934 & 0.024 \\
2455079.77503 & 11.910 & 0.025 \\
2455079.98352 & 11.928 & 0.026 \\
2455081.76585 & 11.844 & 0.042 \\
2455082.99407 & 11.935 & 0.030 \\
2455088.79502 & 11.950 & 0.034 \\
2455097.72923 & 11.900 & 0.033 \\
2455097.93098 & 11.920 & 0.029 \\
2455098.72836 & 11.831 & 0.026 \\
2455098.91806 & 11.934 & 0.034 \\
2455102.76347 & 11.902 & 0.030 \\
2455103.75352 & 11.933 & 0.034 \\
2455103.90449 & 11.921 & 0.033 \\
2455104.75497 & 11.935 & 0.035 \\
2455104.93190 & 11.939 & 0.036 \\
2455105.73253 & 11.909 & 0.030 \\
2455106.72624 & 11.924 & 0.034 \\
2455106.93215 & 11.884 & 0.023 \\
2455112.83804 & 11.919 & 0.030 \\
2455113.84426 & 11.969 & 0.028 \\
2455114.74447 & 11.901 & 0.032 \\
2455115.72396 & 11.944 & 0.032 \\
2455116.72468 & 11.894 & 0.032 \\
2455117.71413 & 11.955 & 0.034 \\
2455118.71549 & 11.888 & 0.041 \\
2455119.71470 & 11.911 & 0.043 \\
2455120.81408 & 11.902 & 0.042 \\
2455121.76921 & 11.916 & 0.019 \\
2455122.72399 & 11.916 & 0.019 \\
2455123.71409 & 11.949 & 0.030 \\
2455124.83729 & 11.927 & 0.024 \\
2455125.70717 & 11.947 & 0.028 \\
2455126.70903 & 11.926 & 0.026 \\
2455127.74605 & 11.894 & 0.030 \\
2455128.74951 & 11.898 & 0.025 \\
2455153.75044 & 11.912 & 0.018 \\
2455156.73001 & 11.899 & 0.028 \\
2455158.74271 & 11.890 & 0.020 \\
2455160.74857 & 11.930 & 0.025 \\
2455166.72835 & 11.901 & 0.024 \\
2455173.71249 & 11.879 & 0.025 \\
2455176.70511 & 11.922 & 0.029 \\
2455179.72208 & 11.924 & 0.033 \\
2455181.72268 & 11.893 & 0.029 \\
2455184.70535 & 11.900 & 0.028 \\
2455187.70158 & 11.880 & 0.030 \\
2455257.15969 & 11.935 & 0.025 \\
2455279.13858 & 11.887 & 0.042 \\
2455283.10457 & 11.930 & 0.018 \\
2455304.11313 & 11.922 & 0.026 \\
2455307.07782 & 11.936 & 0.025 \\
2455310.08736 & 11.914 & 0.020 \\
2455314.10501 & 11.908 & 0.022 \\
2455318.03739 & 11.932 & 0.024 \\
2455321.10952 & 11.910 & 0.017 \\
2455324.10012 & 11.950 & 0.033 \\
2455327.08663 & 11.941 & 0.029 \\
2455330.08869 & 11.903 & 0.025 \\
2455333.08965 & 11.919 & 0.033 \\
2455336.04198 & 11.923 & 0.026 \\
2455343.02404 & 11.935 & 0.023 \\
2455346.01419 & 11.954 & 0.021 \\
2455349.03455 & 11.905 & 0.022 \\
2455352.01509 & 11.902 & 0.024 \\
2455355.00983 & 11.915 & 0.028 \\
2455359.01216 & 11.898 & 0.023 \\
2455362.00947 & 11.916 & 0.026 \\
2455364.03073 & 11.915 & 0.019 \\
2455366.02124 & 11.896 & 0.024 \\
2455368.98059 & 11.885 & 0.029 \\
2455371.02225 & 11.922 & 0.024 \\
2455373.98910 & 11.919 & 0.024 \\
2455376.02241 & 11.929 & 0.021 \\
2455378.04235 & 11.907 & 0.034 \\
2455380.01982 & 11.941 & 0.026 \\
2455382.93940 & 11.928 & 0.037 \\
2455384.99143 & 11.924 & 0.027 \\
2455393.96605 & 11.912 & 0.025 \\
2455396.95672 & 11.927 & 0.019 \\
2455399.01046 & 11.939 & 0.027 \\
2455401.89630 & 11.936 & 0.020 \\
2455403.93438 & 11.915 & 0.020 \\
2455405.93908 & 11.967 & 0.036 \\
2455407.94018 & 11.937 & 0.025 \\
2455411.97063 & 11.882 & 0.028 \\
2455413.93768 & 11.925 & 0.025 \\
2455416.94075 & 11.908 & 0.023 \\
2455418.97952 & 11.945 & 0.025 \\
2455421.88996 & 11.936 & 0.024 \\
2455423.94094 & 11.902 & 0.023 \\
2455425.90761 & 11.912 & 0.026 \\
2455427.87306 & 11.951 & 0.020 \\
2455429.88494 & 11.934 & 0.027 \\
2455432.79856 & 11.930 & 0.029 \\
2455437.88100 & 11.916 & 0.022 \\
2455439.87766 & 11.907 & 0.027 \\
2455441.87488 & 11.894 & 0.034 \\
2455443.86891 & 11.934 & 0.033 \\
2455445.86852 & 11.945 & 0.019 \\
2455447.90192 & 11.923 & 0.029 \\
2455449.93158 & 11.868 & 0.034 \\
2455451.96667 & 11.948 & 0.023 \\
2455453.84768 & 11.903 & 0.029 \\
2455455.82120 & 11.916 & 0.021 \\
2455457.82415 & 11.909 & 0.024 \\
2455460.90992 & 11.891 & 0.033 \\
2455463.87848 & 11.935 & 0.034 \\
2455465.87153 & 11.938 & 0.035 \\
2455472.91156 & 11.947 & 0.023 \\
2455475.85756 & 11.917 & 0.021 \\
2455477.89247 & 11.943 & 0.028 \\
2455479.89223 & 11.930 & 0.026 \\
2455481.86942 & 11.953 & 0.025 \\
2455483.85446 & 11.911 & 0.029 \\
2455486.73878 & 11.934 & 0.032 \\
2455489.82653 & 11.952 & 0.022 \\
2455492.84762 & 11.937 & 0.034 \\
2455501.83352 & 11.911 & 0.029 \\
2455503.80173 & 11.942 & 0.027 \\
2455507.80990 & 11.898 & 0.027 \\
2455509.80742 & 11.931 & 0.028 \\
2455511.81272 & 12.010 & 0.033 \\
2455514.74313 & 11.929 & 0.021 \\
2455517.79078 & 11.884 & 0.023 \\
2455522.69581 & 11.939 & 0.038 \\
2455527.72342 & 11.922 & 0.018 \\
2455535.74415 & 11.928 & 0.023 \\
2455538.70812 & 11.907 & 0.024 \\
2455614.16836 & 11.864 & 0.028 \\
2455621.16839 & 12.061 & 0.032 \\
2455634.16095 & 11.981 & 0.039 \\
2455637.14823 & 11.928 & 0.021 \\
2455644.12817 & 11.934 & 0.017 \\
2455653.13420 & 11.914 & 0.024 \\
2455656.13765 & 11.911 & 0.029 \\
2455664.10785 & 11.930 & 0.028 \\
2455667.08682 & 11.905 & 0.038 \\
2455673.07002 & 11.922 & 0.042 \\
2455680.07298 & 11.897 & 0.028 \\
2455697.07011 & 11.939 & 0.030 \\
2455700.03039 & 11.953 & 0.028 \\
2455706.07128 & 11.939 & 0.025 \\
2455710.01558 & 11.945 & 0.022 \\
2455713.03896 & 11.921 & 0.026 \\
2455719.07381 & 11.914 & 0.026 \\
2455721.05609 & 11.952 & 0.023 \\
2455723.00581 & 11.985 & 0.031 \\
2455725.01171 & 11.985 & 0.030 \\
2455727.06054 & 11.961 & 0.036 \\
2455731.10966 & 11.920 & 0.023 \\
2455743.01029 & 11.940 & 0.027 \\
2455750.99736 & 11.908 & 0.020 \\
2455753.01117 & 11.925 & 0.019 \\
2455759.94974 & 11.921 & 0.028 \\
2455761.96121 & 11.947 & 0.023 \\
2455763.96772 & 11.929 & 0.022 \\
2455766.03648 & 11.915 & 0.023 \\
2455768.87843 & 11.947 & 0.022 \\
2455770.93224 & 11.975 & 0.025 \\
2455773.99231 & 11.917 & 0.031 \\
2455776.04217 & 11.904 & 0.029 \\
2455777.97165 & 11.957 & 0.027 \\
2455779.97897 & 11.942 & 0.024 \\
2455783.08340 & 11.920 & 0.030 \\
2455785.90615 & 12.024 & 0.039 \\
2455787.97199 & 11.941 & 0.030 \\
2455789.94193 & 11.890 & 0.025 \\
2455791.95215 & 11.906 & 0.028 \\
2455793.94909 & 11.950 & 0.030 \\
2455796.80484 & 11.949 & 0.028 \\
2455798.89204 & 11.953 & 0.028 \\
2455801.87152 & 11.942 & 0.021 \\
2455803.90535 & 11.936 & 0.024 \\
2455818.84534 & 11.902 & 0.027 \\
2455821.87928 & 11.948 & 0.031 \\
2455823.85643 & 11.955 & 0.029 \\
2455825.86208 & 11.951 & 0.028 \\
2455827.87215 & 11.951 & 0.026 \\
2455829.87487 & 11.895 & 0.027 \\
2455831.87354 & 11.921 & 0.027 \\
2455835.85262 & 11.917 & 0.028 \\
2455837.84764 & 11.951 & 0.029 \\
2455840.79170 & 11.989 & 0.029 \\
2455844.86082 & 11.960 & 0.027 \\
2455846.87305 & 11.901 & 0.029 \\
2455848.87158 & 11.940 & 0.024 \\
2455851.87183 & 11.918 & 0.026 \\
2455853.87191 & 11.960 & 0.034 \\
2455855.86967 & 11.968 & 0.027 \\
2455858.76835 & 11.914 & 0.038 \\
2455860.79633 & 11.919 & 0.022 \\
2455877.81466 & 11.905 & 0.026 \\
2455880.77135 & 11.918 & 0.032 \\
2455882.78986 & 11.938 & 0.043 \\
2455888.70000 & 11.901 & 0.021 \\
2455894.74083 & 11.925 & 0.022 \\
2455896.74985 & 11.971 & 0.026 \\
2455904.71463 & 11.876 & 0.033 \\
2455911.72743 & 11.935 & 0.030 \\
2455918.69832 & 11.933 & 0.027 \\
2455986.16569 & 12.021 & 0.042 \\
2456001.15702 & 11.992 & 0.033 \\
2456007.14160 & 11.934 & 0.018 \\
2456016.09686 & 11.927 & 0.032 \\
2456020.11120 & 11.948 & 0.033 \\
2456029.08677 & 11.932 & 0.032 \\
2456032.10696 & 11.962 & 0.028 \\
2456039.09752 & 11.941 & 0.030 \\
2456042.05711 & 12.007 & 0.035 \\
2456045.08161 & 11.955 & 0.025 \\
2456064.08759 & 11.962 & 0.024 \\
2456067.06026 & 11.947 & 0.025 \\
2456070.06578 & 11.938 & 0.027 \\
2456073.05744 & 11.977 & 0.026 \\
2456077.07909 & 11.963 & 0.020 \\
2456080.02305 & 11.949 & 0.024 \\
2456083.01194 & 11.968 & 0.021 \\
2456086.01388 & 11.993 & 0.032 \\
2456088.05391 & 11.989 & 0.025 \\
2456093.98240 & 11.964 & 0.022 \\
2456125.97081 & 11.966 & 0.023 \\
2456127.98719 & 11.952 & 0.024 \\
2456135.95081 & 11.963 & 0.024 \\
2456137.92936 & 11.972 & 0.026 \\
2456140.95054 & 11.939 & 0.025 \\
2456142.97685 & 11.948 & 0.031 \\
2456144.97167 & 11.945 & 0.031 \\
2456146.98265 & 11.969 & 0.029 \\
2456148.97304 & 11.952 & 0.025 \\
2456150.97017 & 11.950 & 0.025 \\
2456152.99616 & 11.971 & 0.020 \\
2456155.01904 & 11.969 & 0.023 \\
2456157.02124 & 11.973 & 0.024 \\
2456160.90055 & 11.945 & 0.022 \\
2456162.97139 & 11.968 & 0.027 \\
2456176.81644 & 11.954 & 0.029 \\
2456181.85066 & 11.987 & 0.026 \\
2456183.86777 & 11.946 & 0.027 \\
2456185.87195 & 11.953 & 0.024 \\
2456187.87321 & 12.023 & 0.028 \\
2456192.77692 & 11.959 & 0.025 \\
2456193.93334 & 11.960 & 0.024 \\
2456196.85907 & 11.890 & 0.024 \\
2456200.90230 & 11.933 & 0.033 \\
2456204.81919 & 11.982 & 0.030 \\
2456206.84163 & 11.940 & 0.023 \\
2456208.83963 & 11.945 & 0.023 \\
2456210.83620 & 11.963 & 0.025 \\
2456212.83599 & 11.973 & 0.021 \\
2456214.82999 & 11.947 & 0.024 \\
2456216.82493 & 12.005 & 0.023 \\
2456218.80791 & 11.954 & 0.029 \\
2456220.79005 & 11.969 & 0.031 \\
2456222.80869 & 11.963 & 0.026 \\
2456224.83703 & 11.968 & 0.031 \\
2456227.84212 & 11.965 & 0.032 \\
2456229.83906 & 11.961 & 0.028 \\
2456231.83007 & 11.996 & 0.035 \\
2456233.83007 & 11.964 & 0.033 \\
2456235.83029 & 11.973 & 0.036 \\
2456239.82937 & 11.936 & 0.034 \\
2456242.75390 & 11.942 & 0.023 \\
2456246.76432 & 11.982 & 0.032 \\
2456259.71392 & 11.967 & 0.027 \\
2456268.69705 & 11.964 & 0.031 \\
2456272.69833 & 11.962 & 0.027 \\
2456276.69944 & 11.962 & 0.024 \\
2456354.16007 & 11.953 & 0.027 \\
2456358.15242 & 11.999 & 0.024 \\
2456380.14657 & 12.012 & 0.034 \\
2456388.12338 & 11.903 & 0.037 \\
2456393.12755 & 11.965 & 0.028 \\
2456396.10671 & 11.965 & 0.033 \\
2456399.08479 & 11.977 & 0.035 \\
2456402.07324 & 11.936 & 0.031 \\
2456405.06210 & 11.936 & 0.029 \\
2456408.09338 & 11.988 & 0.034 \\
2456415.09088 & 11.966 & 0.033 \\
2456436.10459 & 11.927 & 0.028 \\
2456443.08970 & 11.952 & 0.029 \\
2456486.12067 & 11.939 & 0.029 \\
2456488.02178 & 11.936 & 0.032 \\
2456490.90526 & 11.982 & 0.030 \\
2456492.94652 & 11.954 & 0.024 \\
2456498.01381 & 12.040 & 0.031 \\
2456525.93400 & 11.913 & 0.034 \\
2456527.93345 & 11.932 & 0.032 \\
2456531.95105 & 11.939 & 0.032 \\
2456533.95002 & 11.968 & 0.039 \\
2456535.94268 & 11.954 & 0.034 \\
2456537.95821 & 11.954 & 0.030 \\
2456540.01305 & 11.989 & 0.039 \\
2456558.78925 & 11.997 & 0.030 \\
2456562.78709 & 11.958 & 0.029 \\
2456564.92529 & 11.967 & 0.027 \\
2456568.83787 & 11.975 & 0.045 \\
2456570.85824 & 11.993 & 0.030 \\
2456577.84350 & 11.953 & 0.037 \\
2456582.83991 & 11.994 & 0.040 \\
2456585.82999 & 11.972 & 0.041 \\
2456587.83009 & 12.035 & 0.039 \\
2456589.85769 & 11.996 & 0.033 \\
2456593.75715 & 11.980 & 0.040 \\
2456597.75840 & 11.936 & 0.024 \\
2456613.76326 & 12.006 & 0.031 \\
2456615.78993 & 11.958 & 0.026 \\
2456618.77656 & 11.938 & 0.024 \\
2456621.77268 & 11.975 & 0.029 \\
2456632.74818 & 12.002 & 0.031 \\
2456637.71908 & 11.969 & 0.028 \\
2456652.69599 & 11.940 & 0.028 \\
2456810.08635 & 11.876 & 0.026 \\
2456813.01287 & 11.901 & 0.027 \\
2456815.95251 & 11.955 & 0.033 \\
2456817.99168 & 11.947 & 0.027 \\
2456854.04145 & 11.946 & 0.033 \\
2456856.02795 & 11.940 & 0.031 \\
2456859.94807 & 12.006 & 0.034 \\
2456863.06138 & 11.924 & 0.025 \\
2456865.88518 & 11.916 & 0.031 \\
2456867.92403 & 11.892 & 0.031 \\
2456869.94057 & 11.941 & 0.035 \\
2456873.94143 & 11.929 & 0.030 \\
2456875.91697 & 11.918 & 0.027 \\
2456883.88485 & 11.963 & 0.025 \\
2456885.96419 & 11.890 & 0.027 \\
2456887.93003 & 11.943 & 0.027 \\
2456892.80585 & 11.931 & 0.030 \\
2456895.90065 & 11.904 & 0.028 \\
2456897.88957 & 11.884 & 0.034 \\
2456900.85203 & 11.929 & 0.027 \\
2456903.00770 & 11.964 & 0.034 \\
2456906.86493 & 11.948 & 0.031 \\
2456913.80418 & 11.940 & 0.032 \\
2456915.84623 & 11.957 & 0.028 \\
2456918.79049 & 11.969 & 0.029 \\
2457081.15953 & 11.918 & 0.030 \\
2457097.15392 & 11.930 & 0.031 \\
2457101.14041 & 11.926 & 0.032 \\
2457110.11112 & 11.908 & 0.028 \\
2457114.11179 & 11.874 & 0.026 \\
2457119.12100 & 11.887 & 0.026 \\
2457122.12334 & 11.940 & 0.038 \\
2457126.13346 & 11.947 & 0.035 \\
2457172.09370 & 11.917 & 0.033 \\
2457180.07402 & 11.916 & 0.033 \\
2457183.06701 & 11.904 & 0.033 \\
2457466.13731 & 11.936 & 0.029 \\
2457479.11300 & 11.930 & 0.029 \\
2457493.11668 & 11.965 & 0.024 \\
2457498.12198 & 11.964 & 0.038 \\
2457506.05802 & 12.022 & 0.029 \\
2457515.03369 & 11.982 & 0.037 \\
2457532.10553 & 11.924 & 0.027 \\
2457536.10765 & 11.914 & 0.033 \\
2457539.02397 & 11.921 & 0.038 \\
2457543.07008 & 11.935 & 0.033 \\
2457546.99691 & 11.972 & 0.033 \\
2457549.96499 & 11.949 & 0.025 \\
2457555.11126 & 11.922 & 0.029 \\
2457557.98800 & 11.923 & 0.029 \\
2457559.97113 & 11.944 & 0.033 \\
2457562.04220 & 11.946 & 0.035 \\
2457568.94463 & 11.916 & 0.039 \\
2457573.99319 & 11.936 & 0.024 \\
2457591.99523 & 11.957 & 0.032 \\
2457595.94710 & 11.911 & 0.027 \\
2457597.96060 & 11.909 & 0.025 \\
2457600.92755 & 11.965 & 0.033 \\
2457603.00321 & 11.944 & 0.032 \\
2457605.85587 & 11.941 & 0.022 \\
2457607.90384 & 12.009 & 0.040 \\
2457609.91922 & 11.934 & 0.030 \\
2457611.89396 & 11.951 & 0.028 \\
2457613.87983 & 11.970 & 0.036 \\
2457616.89907 & 11.910 & 0.031 \\
2457618.93532 & 11.879 & 0.032 \\
2457621.83928 & 11.934 & 0.028 \\
2457625.85687 & 11.965 & 0.030 \\
2457627.86340 & 11.925 & 0.035 \\
2457636.87165 & 11.931 & 0.029 \\
2457643.87838 & 11.903 & 0.037 \\
2457649.86555 & 11.955 & 0.037 \\
2457656.78321 & 11.934 & 0.028 \\
2457658.81726 & 11.935 & 0.026 \\
2457661.91772 & 11.917 & 0.031 \\
2457667.76661 & 11.969 & 0.034 \\
2457669.78641 & 11.906 & 0.039 \\
2457671.79499 & 11.959 & 0.039 \\
2457673.82397 & 11.940 & 0.028 \\
2457687.80680 & 11.960 & 0.033 \\
2457689.82235 & 11.948 & 0.027 \\
2457692.78393 & 11.918 & 0.025 \\
2457701.71762 & 12.002 & 0.025 \\
2457703.79920 & 11.905 & 0.026 \\
2457709.70952 & 11.955 & 0.026 \\
2457715.69706 & 11.948 & 0.023 \\
2457832.13737 & 11.924 & 0.027 \\
2457870.08992 & 11.955 & 0.026 \\
2457879.01367 & 11.919 & 0.031 \\
2457883.09430 & 11.908 & 0.031 \\
2457886.08706 & 11.961 & 0.030 
\enddata
\label{asas_data_table}
\end{deluxetable}


==> asassn_data_table.tex <==
\begin{deluxetable}{lcccc}
\tablecaption{ASAS-SN Photometry of Boyajian's Star}
\tablewidth{0pt}
\tablehead{
\colhead{HJD} &
\colhead{$V$} &
\colhead{$\DeltaV$} & 
\colhead{FWHM} &
\colhead{Zero point\tablenotemark{a}} \\
\colhead{} &
\colhead{[mag]} &
\colhead{[mag]} &
\colhead{[pix]} &
\colhead{[mag]}
}
\startdata
2457078.15792 & 11.898 & 0.009 & 1.56 & -2.26 \\
2457079.15672 & 11.888 & 0.010 & 1.65 & -2.27 \\
2457080.15999 & 11.903 & 0.010 & 1.50 & -2.24 \\
2457081.16257 & 11.894 & 0.011 & 1.69 & -2.25 \\
2457083.16491 & 11.882 & 0.012 & 1.73 & -2.25 \\
2457084.16041 & 11.924 & 0.011 & 2.12 & -2.26 \\
2457103.14733 & 11.910 & 0.010 & 1.51 & -2.20 \\
2457106.11872 & 11.912 & 0.010 & 1.54 & -2.22 \\
2457107.13016 & 11.899 & 0.009 & 1.47 & -2.26 \\
2457114.09387 & 11.902 & 0.010 & 1.66 & -2.26 \\
2457115.09692 & 11.899 & 0.010 & 1.76 & -2.24 \\
2457136.09132 & 11.890 & 0.008 & 1.56 & -2.19 \\
2457137.03437 & 11.893 & 0.009 & 1.48 & -2.24 \\
2457138.05246 & 11.910 & 0.009 & 1.76 & -2.22 \\
2457155.99493 & 11.896 & 0.009 & 1.66 & -2.27 \\
2457162.03376 & 11.915 & 0.010 & 1.52 & -2.32 \\
2457163.00383 & 11.907 & 0.010 & 1.56 & -2.21 \\
2457167.02429 & 11.903 & 0.010 & 1.51 & -2.19 \\
2457172.93225 & 11.903 & 0.009 & 1.43 & -2.23 \\
2457180.04061 & 11.901 & 0.009 & 1.69 & -2.17 \\
2457181.92106 & 11.899 & 0.009 & 1.53 & -2.23 \\
2457183.94537 & 11.927 & 0.010 & 1.62 & -2.20 \\
2457190.93745 & 11.907 & 0.010 & 2.05 & -2.35 \\
2457192.98588 & 11.910 & 0.009 & 1.47 & -2.19 \\
2457199.85992 & 11.919 & 0.010 & 1.48 & -2.24 \\
2457200.01012 & 11.900 & 0.009 & 1.51 & -2.19 \\
2457203.84398 & 11.903 & 0.010 & 1.63 & -2.25 \\
2457210.01666 & 11.882 & 0.009 & 1.65 & -2.20 \\
2457213.02163 & 11.906 & 0.009 & 1.64 & -2.20 \\
2457217.87128 & 11.916 & 0.010 & 1.49 & -2.31 \\
2457218.96076 & 11.904 & 0.009 & 1.66 & -2.18 \\
2457226.82593 & 11.889 & 0.009 & 1.69 & -2.23 \\
2457233.02481 & 11.907 & 0.009 & 1.55 & -2.17 \\
2457235.74961 & 11.932 & 0.011 & 1.67 & -2.21 \\
2457237.81861 & 11.905 & 0.009 & 1.45 & -2.16 \\
2457241.97213 & 11.896 & 0.009 & 1.54 & -2.17 \\
2457243.91135 & 11.905 & 0.009 & 1.49 & -2.15 \\
2457244.76638 & 11.895 & 0.009 & 1.80 & -2.21 \\
2457255.87552 & 11.905 & 0.009 & 1.61 & -2.19 \\
2457263.81821 & 11.900 & 0.011 & 1.52 & -2.29 \\
2457265.93271 & 11.906 & 0.009 & 1.50 & -2.18 \\
2457270.87523 & 11.898 & 0.010 & 1.56 & -2.64 \\
2457271.72880 & 11.894 & 0.009 & 1.54 & -2.19 \\
2457273.91178 & 11.899 & 0.009 & 1.46 & -2.20 \\
2457277.90061 & 11.901 & 0.009 & 1.48 & -2.20 \\
2457296.84558 & 11.890 & 0.009 & 1.57 & -2.20 \\
2457298.84454 & 11.904 & 0.010 & 1.60 & -2.21 \\
2457300.83735 & 11.917 & 0.009 & 1.48 & -2.32 \\
2457303.75425 & 11.916 & 0.009 & 1.67 & -2.17 \\
2457308.76515 & 11.915 & 0.009 & 1.51 & -2.18 \\
2457314.79646 & 11.898 & 0.010 & 1.51 & -2.65 \\
2457318.75486 & 11.919 & 0.010 & 1.49 & -2.20 \\
2457320.69534 & 11.887 & 0.010 & 1.85 & -2.20 \\
2457322.71593 & 11.903 & 0.011 & 1.63 & -2.25 \\
2457324.74959 & 11.892 & 0.010 & 1.52 & -2.22 \\
2457328.75058 & 11.915 & 0.011 & 1.56 & -2.47 \\
2457330.75332 & 11.893 & 0.009 & 1.70 & -2.22 \\
2457333.72841 & 11.906 & 0.010 & 1.60 & -2.19 \\
2457449.16293 & 11.909 & 0.012 & 1.59 & -2.22 \\
2457450.15563 & 11.905 & 0.009 & 1.54 & -2.23 \\
2457452.14857 & 11.887 & 0.009 & 1.50 & -2.24 \\
2457455.14161 & 11.896 & 0.010 & 1.67 & -2.70 \\
2457457.14074 & 11.891 & 0.012 & 1.60 & -2.99 \\
2457457.16116 & 11.859 & 0.013 & 1.69 & -2.66 \\
2457458.13591 & 11.905 & 0.009 & 1.59 & -2.24 \\
2457465.12771 & 11.924 & 0.010 & 1.60 & -2.24 \\
2457467.12652 & 11.897 & 0.011 & 1.60 & -2.68 \\
2457470.11368 & 11.904 & 0.011 & 1.64 & -2.44 \\
2457475.10370 & 11.911 & 0.010 & 1.63 & -2.26 \\
2457481.10780 & 11.914 & 0.009 & 1.80 & -2.22 \\
2457488.08176 & 11.908 & 0.009 & 1.52 & -2.25 \\
2457494.06601 & 11.913 & 0.009 & 1.67 & -2.25 \\
2457500.07192 & 11.911 & 0.009 & 1.43 & -2.21 \\
2457506.03493 & 11.904 & 0.009 & 1.70 & -2.26 \\
2457508.04421 & 11.898 & 0.009 & 1.98 & -2.26 \\
2457512.06834 & 11.918 & 0.009 & 1.55 & -2.21 \\
2457523.97085 & 11.909 & 0.010 & 1.53 & -2.27 \\
2457526.09793 & 11.906 & 0.009 & 1.53 & -2.22 \\
2457528.95805 & 11.907 & 0.010 & 1.55 & -2.29 \\
2457536.07566 & 11.925 & 0.010 & 1.51 & -2.20 \\
2457542.02348 & 11.907 & 0.009 & 1.52 & -2.30 \\
2457548.98016 & 11.902 & 0.008 & 1.46 & -2.21 \\
2457558.98417 & 11.920 & 0.010 & 1.56 & -2.18 \\
2457566.91738 & 11.915 & 0.009 & 1.51 & -2.19 \\
2457570.92402 & 11.898 & 0.009 & 1.67 & -2.21 \\
2457575.99337 & 11.918 & 0.009 & 1.56 & -2.20 \\
2457582.00445 & 11.908 & 0.010 & 1.73 & -2.42 \\
2457582.99273 & 11.916 & 0.010 & 1.59 & -2.20 \\
2457586.91538 & 11.911 & 0.009 & 1.63 & -2.22 \\
2457592.84668 & 11.904 & 0.009 & 1.57 & -2.23 \\
2457596.89232 & 11.917 & 0.009 & 1.70 & -2.21 \\
2457603.01240 & 11.925 & 0.009 & 1.57 & -2.21 \\
2457605.97223 & 11.927 & 0.010 & 2.27 & -2.31 \\
2457606.84673 & 11.925 & 0.010 & 2.09 & -2.28 \\
2457608.90911 & 11.901 & 0.008 & 1.51 & -2.20 \\
2457610.74229 & 11.909 & 0.009 & 1.85 & -2.23 \\
2457611.96791 & 11.909 & 0.009 & 1.47 & -2.21 \\
2457613.75864 & 11.906 & 0.009 & 1.47 & -2.22 \\
2457617.96356 & 11.888 & 0.009 & 1.44 & -2.21 \\
2457620.81107 & 11.899 & 0.009 & 1.65 & -2.20 \\
2457625.81490 & 11.919 & 0.009 & 1.54 & -2.19 \\
2457626.80212 & 11.901 & 0.008 & 1.53 & -2.22 \\
2457636.91479 & 11.913 & 0.010 & 1.53 & -2.22 \\
2457638.86093 & 11.915 & 0.009 & 1.56 & -2.21 \\
2457643.84120 & 11.911 & 0.009 & 1.50 & -2.25 \\
2457652.87001 & 11.902 & 0.010 & 1.64 & -2.24 \\
2457656.81132 & 11.909 & 0.010 & 1.55 & -2.22 \\
2457659.87387 & 11.912 & 0.010 & 1.80 & -2.25 \\
2457662.77707 & 11.933 & 0.010 & 1.55 & -2.24 \\
2457668.82813 & 11.919 & 0.010 & 1.56 & -2.22 \\
2457671.78874 & 11.909 & 0.010 & 1.52 & -2.34 \\
\enddata
\tablenotetext{a}{The ASAS-SN zero point (ZP) of each image
is defined such that a source with a flux of one count has a
magnitude of $25 + \textrm{ZP}$.}
\label{asassn_data_table}
\end{deluxetable}

